NASS: Optimizing Secure Inference via Neural Architecture Search

Due to increasing privacy concerns, neural network (NN) based secure inference (SI) schemes that simultaneously hide the client inputs and server models attract major research interests. While existing works focused on developing secure protocols for NN-based SI, in this work, we take a different approach. We propose NASS, an integrated framework to search for tailored NN architectures designed specifically for SI. In particular, we propose to model cryptographic protocols as design elements with associated reward functions. The characterized models are then adopted in a joint optimization with predicted hyperparameters in identifying the best NN architectures that balance prediction accuracy and execution efficiency. In the experiment, it is demonstrated that we can achieve the best of both worlds by using NASS, where the prediction accuracy can be improved from 81.6% to 84.6%, while the inference runtime is reduced by 2x and communication bandwidth by 1.9x on the CIFAR-10 dataset.

==> rebuttal/rebuttal.tex <==
Reviewer 1
Thank you for your questions. 
Question 1:
What are free (hyper)-parameters of the method they present in the
paper? What NN architectures are they able to evolve? Where are inherent
limits of the approach?
Answer 1:
 i) Several sets of hyper-parameters are introduced according
 to different parts of NASS.
 First, the main hyper-parameters for the NAS engine are
 the input and filter quantizers, filter dimensions, channels (defined by the 
 LayerParms variable in the manuscript)  and $SW_{N}$. These parameters define 
 the architectural search space.
 Second, for cryptography, we need the pre-defined security level and decryption 
 failure rate (delta). 
 Finally, we use beta and gamma to adjust the impact of the rewards throughout the 
 learning process of the NASS controller.
 ii) NASS is a general framework which can be easily configured to support 
 different architectures, as long as they can be implemented by the secure protocols.
 The secure protocols (garbled circuits and homomorphic encryption) used in NASS 
 permit arbitrary function evaluations, so NASS can target a broad set of backbone 
 architectures.  In the experiments, we apply a VGG-like network as the backbone for 
 the architecture search.
 iii) We think that the main limitation to NAS for secure inference (SI) is the fact that it is
 hard to automate the process of secure protocol design.
 In NASS, many cryptographic primitives (e.g., homomorphic encryption, garbled circuits, 
 and secret sharing) are used. There are actually a lot of ways to combine these 
 primitives together as a protocol to carry out the same computations involved in 
 evaluating neural networks securely.  NASS represents the first try to improve the level 
 of automation for secure protocol designs, but there are definitely more works to be 
 done in this field of study.

Question 2:
Do you have idea about the efficiency of the optimization procedure
for the cryptographic part only? Can it be estimated by comparing to
some fixed architecture baseline?
Answer 2:
 i)  On average, generating a set of acceptable parameters for the cryptographic
 primitives takes around 2 to 3 seconds per layer.
 This is considered fast when compared to the process of training the child network.
 In NASS, it takes an average of five minutes to train the child network on the 
 CIFAR-10 dataset.
 ii) Since all existing secure inference schemes use hand-tuned cryptographic parameters (this
 is because they do not need to automate this process for NAS),
 there is no simple benchmark that we can directly compare to. However, as mentioned, the 
 optimization time is fast when compared to the main computational bottleneck in NASS.

REVIEW 3
Thank you for your questions. We intend to publish our codes along with the searched
architectures.
Question 1:
 Please report the computational time for the architecture search.
Answer 1:
 We summarized the overall NASS search time in the rightmost column in Table 1.
 We observe that more than 90% of the reported time is consumed by the repeated 
 training of the child networks.
 
Question 2:
 The authors should review the works of the multiobjective NAS to make
 clear the contribution of the paper.
Answer 2:
 Different from general multi-objective NAS techniques
 suggested by the reviewer, there are two main challenge involved in NASS. First,
 it was not clear if cryptographic primitives can be automatically characterized to
 provide feedbacks for NAS.
 Second, since these primitives have complicated performance curves (as shown in Fig. 1), 
 no existing works demonstrated that
 a multi-objective NAS engine is able to learn the complex behavior
 of the cryptographic primitives (as illustrated in Fig. 5).
 Therefore, the main contribution of NASS is to propose techniques that are integrated 
 into a framework to enable the search for better neural architectures under the context
 of cryptography. We also kindly note that it can be highly non-trivial to adopt 
 some of the existing NAS techniques in NASS (e.g., the techniques from Elsken et al. 
 and Saito et al.) due to the extremely non-linear search spaces of the cryptographic 
 primitives.
